Construction and application of an algebraic dual basis and the Fine-Scale Greens' Function for computing projections and reconstructing unresolved scales

In this paper, we build on the work of [T. Hughes, G. Sangalli, VARIATIONAL MULTISCALE ANALYSIS: THE FINE-SCALE GREENS' FUNCTION, PROJECTION, OPTIMIZATION, LOCALIZATION, AND STABILIZED METHODS, SIAM Journal of Numerical Analysis, 45(2), 2007] dealing with the explicit computation of the Fine-Scale Green's function. The original approach chooses a set of functionals associated with a projector to compute the Fine-Scale Green's function. The construction of these functionals, however, does not generalise to arbitrary projections, higher dimensions, or Spectral Element methods. We propose to generalise the construction of the required functionals by using dual functions. These dual functions can be directly derived from the chosen projector and are explicitly computable. We show how to find the dual functions for both the $L^2$ and the $H^1_0$ projections. We then go on to demonstrate that the Fine-Scale Green's functions constructed with the dual basis functions consistently reproduce the unresolved scales removed by the projector. The methodology is tested using one-dimensional Poisson and advection-diffusion problems, as well as a two-dimensional Poisson problem. We present the computed components of the Fine-Scale Green's function, and the Fine-Scale Green's function itself. These results show that the method works for arbitrary projections, in arbitrary dimensions. Moreover, the methodology can be applied to any Finite/Spectral Element or Isogeometric framework.

==> Images/TikZ/deRhamDisc.tex <==
\begin{tikzpicture}
    \tikzmath{\spacing = 2.12; \hSep = 1.5; \hArrMargin = 0.5; \vArrMargin = 0.4;}
    \coordinate (topLeft) at (0, 0);
    \coordinate (form0) at ($(topLeft) + (\spacing, 0)$);
    \coordinate (form1) at ($(form0) + (\spacing, 0)$);
    \coordinate (form2) at ($(form1) + (\spacing, 0)$);
    \coordinate (zero) at ($(form2) + (\spacing, 0)$);
    \coordinate (botRight) at ($(zero) - (0, \hSep)$);
    \coordinate (formt2) at ($(form0) - (0, \hSep)$);
    \coordinate (formt1) at ($(form1) - (0, \hSep)$);
    \coordinate (formt0) at ($(form2) - (0, \hSep)$);
    \coordinate (zerot) at ($(topLeft) - (0, \hSep)$);
    
    \draw (topLeft) node {$\mathbb{R}$};
    \draw (form0) node {$\Lambda^{(0)}_h$};
    \draw (form1) node {$\Lambda^{(1)}_h$};
    \draw (form2) node {$\Lambda^{(2)}_h$};
    \draw (zero) node {$0$};
    \draw (botRight) node {$\mathbb{R}$};
    \draw (formt0) node {$\tilde{\Lambda}^{(0)}_h$};
    \draw (formt1) node {$\tilde{\Lambda}^{(1)}_h$};
    \draw (formt2) node {$\tilde{\Lambda}^{(2)}_h$};
    \draw (zerot) node {$0$};
    
    \draw[thick, ->] ($(topLeft) + (\hArrMargin/2, 0)$) -- ($(form0) - (\hArrMargin, 0)$);
    \draw[thick, ->] ($(form0) + (\hArrMargin, 0)$) -- ($(form1) - (\hArrMargin, 0)$);
    \draw[thick, ->] ($(form1) + (\hArrMargin, 0)$) -- ($(form2) - (\hArrMargin, 0)$);
    \draw[thick, ->] ($(form2) + (\hArrMargin, 0)$) -- ($(zero) - (\hArrMargin/2, 0)$);
    \draw[thick, ->] ($(botRight) - (\hArrMargin/4, 0)$) -- ($(formt0) + (\hArrMargin, 0)$);
    \draw[thick, ->] ($(formt0) - (\hArrMargin, 0)$) -- ($(formt1) + (\hArrMargin, 0)$);
    \draw[thick, ->] ($(formt1) - (\hArrMargin, 0)$) -- ($(formt2) + (\hArrMargin, 0)$);
    \draw[thick, ->] ($(formt2) - (\hArrMargin, 0)$) -- ($(zerot) + (\hArrMargin/2, 0)$);
    \draw[thick, ->] ($(form0) - (0, \vArrMargin)$) -- ($(formt2) + (0, \vArrMargin)$);
    \draw[thick, ->] ($(form1) - (0, \vArrMargin)$) -- ($(formt1) + (0, \vArrMargin)$);
    \draw[thick, ->] ($(form2) - (0, \vArrMargin)$) -- ($(formt0) + (0, \vArrMargin)$);
    
    \draw ($(form0) + (\spacing/2, \vArrMargin/1.5)$) node {$\E{1}{0}$};
    \draw ($(form1) + (\spacing/2, \vArrMargin/1.5)$) node {$\E{2}{1}$};
    \draw ($(formt0) - (\spacing/2, -\vArrMargin/1.5)$) node {$\tE{1}{0}$};
    \draw ($(formt1) - (\spacing/2, -\vArrMargin/1.5)$) node {$\tE{2}{1}$};
    \draw ($(form0) + (\hArrMargin, -\hSep/2.5)$) node {$\MassM{0}$};
    \draw ($(form1) + (\hArrMargin, -\hSep/2.5)$) node {$\MassM{1}$};
    \draw ($(form2) + (\hArrMargin, -\hSep/2.5)$) node {$\MassM{2}$};
\end{tikzpicture}

==> Images/TikZ/deRhamDisc1D.tex <==
\begin{tikzpicture}
    \tikzmath{\spacing = 2.12; \hSep = 1.5; \hArrMargin = 0.5; \vArrMargin = 0.4;}
    \coordinate (topLeft) at (0, 0);
    \coordinate (form0) at ($(topLeft) + (\spacing, 0)$);
    \coordinate (form1) at ($(form0) + (\spacing, 0)$);
    \coordinate (zero) at ($(form1) + (\spacing, 0)$);
    \coordinate (botRight) at ($(zero) - (0, \hSep)$);
    \coordinate (formt1) at ($(form0) - (0, \hSep)$);
    \coordinate (formt0) at ($(form1) - (0, \hSep)$);
    \coordinate (zerot) at ($(topLeft) - (0, \hSep)$);
    
    \draw (topLeft) node {$\mathbb{R}$};
    \draw (form0) node {$\Lambda^{(0)}_h$};
    \draw (form1) node {$\Lambda^{(1)}_h$};
    \draw (zero) node {$0$};
    \draw (botRight) node {$\mathbb{R}$};
    \draw (formt0) node {$\tilde{\Lambda}^{(0)}_h$};
    \draw (formt1) node {$\tilde{\Lambda}^{(1)}_h$};
    \draw (zerot) node {$0$};
    
    \draw[thick, ->] ($(topLeft) + (\hArrMargin/2, 0)$) -- ($(form0) - (\hArrMargin, 0)$);
    \draw[thick, ->] ($(form0) + (\hArrMargin, 0)$) -- ($(form1) - (\hArrMargin, 0)$);
    \draw[thick, ->] ($(form1) + (\hArrMargin, 0)$) -- ($(zero) - (\hArrMargin/2, 0)$);
    \draw[thick, ->] ($(botRight) - (\hArrMargin/2, 0)$) -- ($(formt0) + (\hArrMargin, 0)$);
    \draw[thick, ->] ($(formt0) - (\hArrMargin, 0)$) -- ($(formt1) + (\hArrMargin, 0)$);
    \draw[thick, ->] ($(formt1) - (\hArrMargin, 0)$) -- ($(zerot) + (\hArrMargin/2, 0)$);
    \draw[thick, ->] ($(form0) - (0, \vArrMargin)$) -- ($(formt1) + (0, \vArrMargin)$);
    \draw[thick, ->] ($(form1) - (0, \vArrMargin)$) -- ($(formt0) + (0, \vArrMargin)$);
    
    \draw ($(form0) + (\spacing/2, \vArrMargin/1.5)$) node {$\E{1}{0}$};
    \draw ($(formt0) - (\spacing/2, -\vArrMargin/1.5)$) node {$\tE{1}{0}$};
    \draw ($(form0) + (\hArrMargin, -\hSep/2.5)$) node {$\MassM{0}$};
    \draw ($(form1) + (\hArrMargin, -\hSep/2.5)$) node {$\MassM{1}$};
\end{tikzpicture}

==> sections/07-recommendations.tex <==
\section{Recommendations}
\label{sec:recommendations}
